A Deep Learning-based Pest Insect Monitoring System for Ultra-low Power Pocket-sized Drones

Smart farming and precision agriculture represent game-changer technologies for efficient and sustainable agribusiness. Miniaturized palm-sized drones can act as flexible smart sensors inspecting crops, looking for early signs of potential pest outbreaking. However, achieving such an ambitious goal requires hardware-software codesign to develop accurate deep learning (DL) detection models while keeping memory and computational needs under an ultra-tight budget, i.e., a few MB on-chip memory and a few 100s mW power envelope. This work presents a novel vertically integrated solution featuring two ultra-low power System-on-Chips (SoCs), i.e., the dual-core STM32H74 and a multi-core GWT GAP9, running two State-of-the-Art DL models for detecting the Popillia japonica bug. We fine-tune both models for our image-based detection task, quantize them in 8-bit integers, and deploy them on the two SoCs. On the STM32H74, we deploy a FOMO-MobileNetV2 model, achieving a mean average precision (mAP) of 0.66 and running at 16.1 frame/s within 498 mW. While on the GAP9 SoC, we deploy a more complex SSDLite-MobileNetV3, which scores an mAP of 0.79 and peaks at 6.8 frame/s within 33 mW. Compared to a top-notch RetinaNet-ResNet101-FPN full-precision baseline, which requires 14.9x more memory and 300x more operations per inference, our best model drops only 15\% in mAP, paving the way toward autonomous palm-sized drones capable of lightweight and precise pest detection.

==> param_count_table.tex <==
\begin{table}[t]
    \small\centering
    \caption{Parameter counts and MACs for the models used in \cite{9601235}. MACs where computed based on  a single RGB input image of size $300\times300$ for SSD models and $800\times800$ for others. Shown numbers are obtained using the torch info python library~\cite{torchinfo} \label{tab:other_models_params}\\}
    
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{llllll}
    \toprule
    \textbf{Network}&\textbf{Input Size}&\textbf{Total Params}&\textbf{GMACs}&\textbf{mAP}&\textbf{Reference}\\
    \toprule
    \textbf{FasterRCNN-VGG16-FPN}&$3\times800\times800$&31,946,595&275.23&0.9242&\cite{FasterRCNN,VGG,FPN}\\
    \midrule
    \textbf{FasterRCNN-ResNet101-FPN}&$3\times800\times800$&60,249,315&167.41&0.9214&\cite{FasterRCNN,ResNet,FPN}\\
    \midrule
    \textbf{FasterRCNN-DenseNet169-FPN}&$3\times800\times800$&30,044,067&73.99&0.9107&\cite{FasterRCNN,DenseNet,FPN}\\
    \midrule
    \textbf{FasterRCNN-MobileNetV3-FPN}&$3\times800\times800$&18,940,479&18.41&0.9266&\cite{FasterRCNN,MobileNetV3,FPN}\\
    \midrule
    \midrule
    \textbf{RetinaNet-VGG16-FPN}&$3\times800\times800$&22,880,136&270.06&0.9125&\cite{RetinaNet,VGG,FPN}\\
    \midrule
    \textbf{RetinaNet-ResNet101-FPN}&$3\times800\times800$&51,150,088&174.85&0.9330&\cite{RetinaNet,ResNet,FPN}\\
    \midrule
    \textbf{RetinaNet-DenseNet169-FPN}&$3\times800\times800$&20,977,608&65.10&0.9170&\cite{RetinaNet,DenseNet,FPN}\\
    \midrule
    \textbf{RetinaNet-MobileNetV3-FPN}&$3\times800\times800$&10,592,344&11.09&0.9066&\cite{RetinaNet,MobileNetV3,FPN}\\
    \midrule
    \midrule
    \textbf{SSD-VGG16}&$3\times300\times300$&12,126,000&26.58&0.5570&\cite{SSD,VGG}\\
    \midrule
    \textbf{SSD-ResNet101}&$3\times300\times300$&32,304,688&42.39&0.8731&\cite{SSD,ResNet}\\
    \midrule
    \textbf{SSD-DenseNet169}&$3\times300\times300$&11,826,800&24.51&0.9238&\cite{SSD,DenseNet}\\
    \midrule
    \textbf{SSD-MobileNetV3}&$3\times300\times300$&7,545,040&3.42&0.8044&\cite{SSD,MobileNetV3}\\
    \bottomrule
    \end{tabular}
    }
\end{table}
